Controllable Human Image Generation with Personalized Multi-Garments

We present BootComp, a novel framework based on text-to-image diffusion models for controllable human image generation with multiple reference garments. Here, the main bottleneck is data acquisition for training: collecting a large-scale dataset of high-quality reference garment images per human subject is quite challenging, i.e., ideally, one needs to manually gather every single garment photograph worn by each human. To address this, we propose a data generation pipeline to construct a large synthetic dataset, consisting of human and multiple-garment pairs, by introducing a model to extract any reference garment images from each human image. To ensure data quality, we also propose a filtering strategy to remove undesirable generated data based on measuring perceptual similarities between the garment presented in human image and extracted garment. Finally, by utilizing the constructed synthetic dataset, we train a diffusion model having two parallel denoising paths that use multiple garment images as conditions to generate human images while preserving their fine-grained details. We further show the wide-applicability of our framework by adapting it to different types of reference-based generation in the fashion domain, including virtual try-on, and controllable human image generation with other conditions, e.g., pose, face, etc.

==> figures/distribution.tex <==
\begin{figure*}[t]
    \small\centering
    \includegraphics[width=0.98\textwidth]{resources/vis_distribution.pdf}
    \vspace{-5pt}
    \caption{\textbf{Comparison between na\"ive distribution merging and bootstrapping based distribution merging.}explanation.} 
    \label{fig:distribution}
    \vspace{-10pt}
\end{figure*}




% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}


==> figures/eg_copy_paste.tex <==
\begin{figure}[!b]
\vspace{-10pt}
\includegraphics[width=\linewidth]{resources/copy_example.pdf}    
% \vspace{-15pt}
\captionof{figure}{\textbf{Limitations of previous methods for compositional generation} While baselines (a) fail to preserve the identity of reference garments and (b) their data generation approaches cause copy-and-paste problem, our methods enable compositional generation.}
% \vspace{-15pt}
\label{fig:example_copy}
\end{figure}

==> figures/reb_limitation.tex <==
\begin{figure}[]
% \vspace{-10pt}
\includegraphics[width=\linewidth]{resources/rebuttal_limitation.pdf}  
% \captionof{figure}{\textbf{Visual comparison of extracted garment.}}
\vspace{-30pt}
% \label{fig:reb_tryoff}
\end{figure}


==> figures/reb_tryoffdiff.tex <==
\begin{figure}[!bh]
\vspace{-15pt}
\includegraphics[width=\linewidth]{resources/rebuttal_decomp_comp.pdf}  
\vspace{-24pt}
% \captionof{figure}{\textbf{Visual comparison of extracted garment.}}
% % \vspace{-15pt}
% \label{fig:reb_tryoff}
\end{figure}


==> figures/reb_vton.tex <==
\begin{figure}[!h]
\vspace{-8pt}
\includegraphics[width=\linewidth]{resources/rebuttal_vton.pdf}  
\vspace{-25pt}
% \captionof{figure}{\textbf{Visual comparison of extracted garment.}}
% % \vspace{-15pt}
% \label{fig:reb_tryoff}
\end{figure}


==> figures/scale.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.7\linewidth]{resources/scaling.pdf}    
\captionof{figure}{\textbf{Scaling the training data} We train our composition module with different scales of data. We see that it shows higher compositionality with the larger training data, demonstrating the scalability of our synthetic data.}
\vspace{-10pt}
\label{fig:scale}
\end{figure}


==> figures/teaser.tex <==

\begin{figure*}[t]
\includegraphics[width=\textwidth, height=0.375\linewidth]{resources/teaser_new.pdf}   
\captionof{figure}{\textbf{Generated images by~\sname}. Given a set of reference garment images,~\sname generates a human image wearing them.
\label{fig:teaser}
\vspace{2em}}
\end{figure*}
